CircuitNet: An Open-Source Dataset for Machine Learning Applications in Electronic Design Automation (EDA)

The electronic design automation (EDA) community has been actively exploring machine learning (ML) for very large-scale integrated computer-aided design (VLSI CAD). Many studies explored learning-based techniques for cross-stage prediction tasks in the design flow to achieve faster design convergence. Although building ML models usually requires a large amount of data, most studies can only generate small internal datasets for validation because of the lack of large public datasets. In this essay, we present the first open-source dataset called CircuitNet for ML tasks in VLSI CAD.

==> texlib/acm_setting.tex <==
% =============================================================
%            settign for ACM format paper
%
%   Author      : Bei Yu
%   Last Update : 12/2014
% =============================================================

\settopmatter{printacmref=false}          % no ACM Reference Format
\fancyhead{}                              % no header

% ==== page margin settings
\geometry{twoside=true, head=13pt,
	paperwidth=8.5in, paperheight=11in,
	includeheadfoot, columnsep=2pc,
	top=45pt, bottom=55pt, 
    left=45pt, right=45pt, 
    %inner=54pt, outer=54pt,
	marginparwidth=2pc,heightrounded
}%
\iffalse
\textfloatsep          = 12pt plus 1pt minus 7pt            % set space between figure and text
\floatsep              = 5pt plus 1pt minus 7pt
\fi
%\intextsep             = 0pt plus 1pt minus 7pt           % set space above and below the texts
%\dbltextfloatsep       = 0pt plus 1pt minus 7pt
%\dblfloatsep           = 0pt plus 1pt minus 7pt
%\abovedisplayskip      = 0pt plus 1pt minus 7pt           % set space around equations
%\belowdisplayskip      = 0pt plus 1pt minus 7pt
%\abovedisplayshortskip = 0pt plus 1pt minus 7pt
%\belowdisplayshortskip = 0pt plus 1pt minus 7pt

% ==== Packages
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{comment}
\usepackage[subrefformat=parens,labelformat=parens]{subfig}
\captionsetup[subfigure]{labelformat=simple}               % avoid "double brackets" in sub-figure caption
\renewcommand\thesubfigure{(\alph{subfigure})}             % "Fig.~1b"-->"Fig.1(b)"
\usepackage{bm}
\usepackage{multirow}
\usepackage{threeparttable,booktabs}
\usepackage{tikz}
\usepackage{balance}
\usepackage{courier}                                       % courier font, used in \texttt
\usepackage{cleveref}                                      % smart citation
%\usepackage[mathcal]{eucal}
%\usepackage[]{algpseudocode}                               % algorithm package
\usepackage[noend]{algpseudocode}
\algrenewcommand\textproc{\texttt}
\makeatletter\let\float@addtolists\relax\makeatother
\usepackage{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:} }       % Use Input in the format of Algorithm
\renewcommand{\algorithmicensure} {\textbf{Output:}}       % Use Output in the format of Algorithm
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{siunitx}
\sisetup{product-units = single}
% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

\theoremstyle{plain}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{myproblem}{\textbf{Problem}}



% ==== spacing control on caption
\usepackage[skip=1pt]{caption}            % set space between figure and caption
\setlength{\belowcaptionskip}{-1.0mm}
\captionsetup[table]{aboveskip=5pt}       % reduce space around table caption
\captionsetup[table]{belowskip=2pt}


==> texlib/ieee_normal.tex <==
% =============================================================
%         setting for IEEE format paper (normal mode)
%
%   Author      : Bei Yu
%   Last Update : 07/2016
% =============================================================


%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}                                 % new algorithm package
\usepackage{algorithm}
\usepackage{graphicx}                                      % include pdf figures
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[subrefformat=parens,farskip=0pt,justification=centering]{subfig}
\usepackage{color}
\usepackage{cite}                                          % more citations in one bracket
\usepackage{comment}                                       % use comment
\usepackage{soul}                                          % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}                                      % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}                                           % nth command
\usepackage{bm}                                            % bm command
\usepackage{balance}
\usepackage{threeparttable}
\usepackage[bookmarks=false]{hyperref}                     %
\hypersetup{
    colorlinks = true,
    citecolor  = blue,
    linkcolor  = blue,
    urlcolor   = blue,
}
\usepackage{filecontents}                                  % support to pgfplots
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\setlength{\columnsep}{18pt}

% =============================================================
%                   Theorem Definitions
% =============================================================
\newtheorem{problem}{\textbf{Problem}}
\newtheorem{definition}{\textbf{Definition}}
\newtheorem{theorem}{\textbf{Theorem}}
\newtheorem{lemma}{\textbf{Lemma}}
\newtheorem{claim}{\textbf{Claim}}
\newtheorem{application}{\textbf{Application}}
\newtheorem{conjecture}{Conjecture}
\newtheorem{prop}{Property}

\algrenewcommand\textproc{\texttt}
\newcommand{\tabincell}[2]{
    \begin{tabular}{@{}#1@{}}#2\end{tabular}
}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% =============================================================
%          Definitions to support latexdiff
% =============================================================
%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}{#1}}}                           %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                       %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFaddend}{}                                                     %DIF PREAMBLE
\providecommand{\DIFdelbegin}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelend}{}                                                     %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                                        %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFaddendFL}{}                                                   %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{}                                                 %DIF PREAMBLE
\providecommand{\DIFdelendFL}{}                                                   %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


% ==== Logs:
%
%  07/2016: support to pgfplots
%  07/2016: threeparttable
%  04/2016: definitions supporting latexdiff
%  04/2016: remove bookmarks in hyperref
%  02/2016: tabincell
%  02/2016: hyperref
%  12/2015: copy from "ieee_conference"
%



==> texlib/ieee_setting.tex <==
% =============================================================
%            setting for IEEE format paper
%
%   Author      : Bei Yu
%   Last Update : 06/2015
% =============================================================


\usepackage[noend]{algpseudocode}
%\usepackage{algpseudocode}    % new algorithm package
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{tikz}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{graphicx}         % include pdf figures
\usepackage{color}
\usepackage{cite}             % more citations in one bracket
\usepackage{comment}          % use comment
\usepackage{soul}             % use highlight command \hl{}
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}         % commands \newtoggle, \toggletrue, \iftoggle
\usepackage{url}
\usepackage{nth}              % nth command
\usepackage{bm}               % bm command
\usepackage{caption} 
\usepackage{subfig}

\usepackage{cleveref}                                      % smart



\theoremstyle{plain}
\newtheorem{theorem}{\textbf{Theorem}}
\newtheorem*{theorem*}{\textbf{Theorem}}
\newtheorem{lemma}{\textbf{Lemma}}
\newtheorem{claim}{\textbf{Claim}}

\theoremstyle{definition}
\newtheorem{definition}{\textbf{Definition}}
\newtheorem{problem}{\textbf{Problem}}
\newtheorem*{problem*}{\textbf{Problem}}


% ==== Local new commands
%\newcommand{\calH}{\mathcal{H}}
%\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
%\newcommand{\calV}{\mathcal{V}}
%\newcommand{\calS}{\mathcal{S}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\vec}[1]{\boldsymbol{#1}} 
%\newcommand{\m}[1]{\mathbf{#1}}
%\newcommand{\mx}{\m{x}}
%\newcommand{\my}{\m{y}}
%\newcommand{\mz}{\m{z}}
\DeclareMathOperator*{\argmin}{argmin}

% long line in algorithm
% e.g.: \Statex[4] ...;
\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


% ==== Logs:
%
%  06/2015: clean IEEEtranBSTCTL commands
%  11/2014: \solregister, to support highlight to mybox, definition, and citations
%  10/2014: add package "authblk" & "bm"
%  09/2014: "problem" => "myproblem"
%  07/2014: introduce \Statex[] for lone algorithmic statement
%  05/2014: new package {soul} to use highlight command \hl{}
%




==> texlib/poster_setting.tex <==
% ============================================================
%             Beamer poster setting file
%
%   Author      : Bei Yu
%   last Update : 06/2014
% ============================================================

% additional settings
\setbeamerfont{itemize}{size=\normalsize}
\setbeamerfont{itemize/enumerate body}{size=\normalsize}
\setbeamerfont{itemize/enumerate subbody}{size=\normalsize}


% block width setting
\newenvironment<>{varblock}[2][\textwidth]{%
  \setlength{\textwidth}{#1}
  \setbeamercolor{block title}{fg=white,bg=blue!20!green}
  %\setbeamercolor{block body}{fg=black,bg=olive!50}
  \setbeamercolor{block body}{fg=black,bg=blue!10}
  \begin{actionenv}#3%
  \def\insertblocktitle{#2}%
  \par%
  \usebeamertemplate{block begin}}
  {
    \par%
    \usebeamertemplate{block end}%
    \end{actionenv}
  }


% abbreviations
\usepackage{xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{{etc}\onedot}
\def\vs{{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{{et al}\onedot}
\makeatother


% === including packages
\usepackage{bm}
\usepackage{xcolor}
\usepackage{colortbl}
\usepackage{times}
\usepackage{amsmath,amsthm, amssymb, latexsym}
\usepackage{exscale}
\usepackage{subfigure}
\usepackage{multirow}
\usepackage{comment}
\usepackage{booktabs, array}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\usepackage[orientation=landscape,size=custom,width=200,height=230,scale=1.9]{beamerposter}
\listfiles

% =====  algorithm setting
%\usepackage[noend]{algpseudocode}
\usepackage{algpseudocode}
\usepackage{algorithm}
%\renewcommand{\algorithmicrequire}{\textbf{Input:}}  % Use Input in the format of Algorithm
%\renewcommand{\algorithmicensure}{\textbf{Output:}} % Use Output in the format of Algorithm

% ==== Log
%
%  05/2014: preliminary results show that pgf library is NOT good for poster
%


